Adaptive norms for deep learning with regularized Newton methods

We investigate the use of regularized Newton methods with adaptive norms for optimizing neural networks. This approach can be seen as a second-order counterpart of adaptive gradient methods, which we here show to be interpretable as first-order trust region methods with ellipsoidal constraints. In particular, we prove that the preconditioning matrix used in RMSProp and Adam satisfies the necessary conditions for provable convergence of second-order trust region methods with standard worst-case complexities on general non-convex objectives. Furthermore, we run experiments across different neural architectures and datasets to find that the ellipsoidal constraints constantly outperform their spherical counterpart both in terms of number of backpropagations and asymptotic loss value. Finally, we find comparable performance to state-of-the-art first-order methods in terms of backpropagations, but further advances in hardware are needed to render Newton methods competitive in terms of computational time.

==> 015_background.tex <==
\section{Background and Notation}
For a symmetric positive definite matrix $\A$ we introduce the compact notation $\|\w\|_\A = \left( \w^\top \A \w \right)^{1/2}$, where $\w \in \mathbb{R}^d$. Then, the notation $\|\w\|_\A  \overset{!}{=}\Delta$ defines an ellipsoid with "radius" delta.

In the easiest case $\A=diag(1/a_1,1/a_2,\ldots,1/a_d)$ the ellipsoid intersects the $i$-th coordinate axis at $\sqrt{a_i}\Delta$. Likewise, dividing a vector by its $\A$-norm , i.e. reparametrizing $\Tilde{\w}:=\w/\|\w\|_\A$ makes $\Tilde{\w}$ live on the $\A$-ellipsoid with $\Delta=1$ in the sense that $\|\Tilde{\w}\|_\A=1$. Finally, off-diagonal elements in $\A$ introduce a shift and stretch effect on the ellipsoid.
